A Complete Approach to Loop Verification with Invariants and Summaries

Invariants are the predominant approach to verify the correctness of loops. As an alternative, loop contracts, which make explicit the premise and conclusion of the underlying induction proof, can sometimes capture correctness conditions more naturally. But despite this advantage, the second approach receives little attention overall, and the goal of this paper is to lift it out of its niche. We give the first comprehensive exposition of the theory of loop contracts, including a characterization of its completeness. We show concrete examples on standard algorithms that showcase their relative merits. Moreover, we demonstrate a novel constructive translation between the two approaches, which decouples the chosen specification approach from the verification backend.

==> figures/steps.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[node distance=2cm]
\node (s0) {$s_0$};
\node (si) [right=2.5cm of s0] {$s_{i}$};
\node (sj) [right=1.5cm of si] {$s_{i+1}$};
\node (sn) [right=2.5cm of sj] {$s_{n}$};

\draw[->,thick,dashed] (s0) -- (si);
\draw[->,thick] (si) -- node[above] {body} (sj);
\draw[->,thick,dashed] (sj) -- (sn);

\node (P0) [above=0.35cm of s0] {$\blue{P(s_0)} \implies \red{I(s_0)}$};
\node (Ii) [above=0.35cm of si] {$\blue{t(s_i) \land I(s_i)}$};
\node (Ij) [above=0.35cm of sj] {$\implies \red{I(s_{i+1})}$};
\node (Qn) [above=0.35cm of sn] {$\blue{\lnot t(s_n)} \implies \red{R(s_n,s_n)}$};

\draw[thick,dotted] (P0) -- (s0);
\draw[thick,dotted] (Ii) -- (si);
\draw[thick,dotted] (Ij) -- (sj);
\draw[thick,dotted] (Qn) -- (sn);

\draw[thick,decorate,decoration={brace,raise=0.3cm,amplitude=2mm,mirror},blue]
    (sj.west) -- (sn.east)
    node [pos=0.5,yshift=-0.8cm] {assume $R(s_{i+1},s_n)$}; ;

\draw[thick,decorate,decoration={brace,raise=1.1cm,amplitude=2mm,mirror},red]
    (si.west) -- (sn.east)
    node [pos=0.5,yshift=-1.6cm] {prove $R(s_i,s_n)$}; ;

\draw[thick,decorate,decoration={brace,raise=1.9cm,amplitude=2mm,mirror},green!70!black]
    (s0.west) -- (sn.east)
    node [pos=0.5,yshift=-2.4cm] {finally $P(s_0) \land R(s_0,s_n) \implies Q(s_n)$}; ;
    \end{tikzpicture}
    \caption{Forward propagation of an invariant~$I$
             and the backward propagation conditions for a summary~$R$
             with respect to an iteration of the loop.
             Assumptions are marked in blue, proof obligations in red,
             and the overall conclusion in green.}
    \label{fig:steps}
\end{figure}



